Direct Estimation of Information Divergence Using Nearest Neighbor Ratios

We propose a direct estimation method for R\'{e}nyi and f-divergence measures based on a new graph theoretical interpretation. Suppose that we are given two sample sets $X$ and $Y$, respectively with $N$ and $M$ samples, where $\eta:=M/N$ is a constant value. Considering the $k$-nearest neighbor ($k$-NN) graph of $Y$ in the joint data set $(X,Y)$, we show that the average powered ratio of the number of $X$ points to the number of $Y$ points among all $k$-NN points is proportional to R\'{e}nyi divergence of $X$ and $Y$ densities. A similar method can also be used to estimate f-divergence measures. We derive bias and variance rates, and show that for the class of $\gamma$-H\"{o}lder smooth functions, the estimator achieves the MSE rate of $O(N^{-2\gamma/(\gamma+d)})$. Furthermore, by using a weighted ensemble estimation technique, for density functions with continuous and bounded derivatives of up to the order $d$, and some extra conditions at the support set boundary, we derive an ensemble estimator that achieves the parametric MSE rate of $O(1/N)$. Our estimators are more computationally tractable than other competing estimators, which makes them appealing in many practical applications.

==> boldLetters.tex <==
%%!TEX TS-program = pdflatex
%%!TEX encoding = UTF-8 Unicode

% 120 Character width (because 80 just wasn't enough)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 80 --> %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 120 -->

% This file provides bold letters under the \b<letterName> syntax.  If a function is already defined under the same
% name and error will be issued

% Some letters may not render as bold if the fonts don't support it

\NewDocumentCommand{\ba}{}{\mbf{a}}
\NewDocumentCommand{\bb}{}{\mbf{b}}
\NewDocumentCommand{\bc}{}{\mbf{c}}
\NewDocumentCommand{\bd}{}{\mbf{d}}
\NewDocumentCommand{\be}{}{\mbf{e}}
%\NewDocumentCommand{\bf}{}{\mbf{f}}  <--- \bf is already "bold face"
\NewDocumentCommand{\bg}{}{\mbf{g}}
\NewDocumentCommand{\bh}{}{\mbf{h}}
\NewDocumentCommand{\bi}{}{\mbf{i}}
\NewDocumentCommand{\bj}{}{\mbf{j}}
\NewDocumentCommand{\bk}{}{\mbf{k}}
\NewDocumentCommand{\bl}{}{\mbf{l}}
%\NewDocumentCommand{\bm}{}{\mbf{m}}  <--- \bm is already "bold math"
\NewDocumentCommand{\bn}{}{\mbf{n}}
\NewDocumentCommand{\bo}{}{\mbf{o}}
\NewDocumentCommand{\bp}{}{\mbf{p}}
\NewDocumentCommand{\bq}{}{\mbf{q}}
\NewDocumentCommand{\br}{}{\mbf{r}}
\NewDocumentCommand{\bs}{}{\mbf{s}}
\NewDocumentCommand{\bt}{}{\mbf{t}}
\NewDocumentCommand{\bu}{}{\mbf{u}}
\NewDocumentCommand{\bv}{}{\mbf{v}}
\NewDocumentCommand{\bw}{}{\mbf{w}}
\NewDocumentCommand{\bx}{}{\mbf{x}}
\NewDocumentCommand{\by}{}{\mbf{y}}
\NewDocumentCommand{\bz}{}{\mbf{z}}

\NewDocumentCommand{\bA}{}{\mbf{A}}
\NewDocumentCommand{\bB}{}{\mbf{B}}
\NewDocumentCommand{\bC}{}{\mbf{C}}
\NewDocumentCommand{\bD}{}{\mbf{D}}
\NewDocumentCommand{\bE}{}{\mbf{E}}
\NewDocumentCommand{\bF}{}{\mbf{F}}
\NewDocumentCommand{\bG}{}{\mbf{G}}
\NewDocumentCommand{\bH}{}{\mbf{H}}
\NewDocumentCommand{\bI}{}{\mbf{I}}
\NewDocumentCommand{\bJ}{}{\mbf{J}}
\NewDocumentCommand{\bK}{}{\mbf{K}}
\NewDocumentCommand{\bL}{}{\mbf{L}}
\NewDocumentCommand{\bM}{}{\mbf{M}}
\NewDocumentCommand{\bN}{}{\mbf{N}}
\NewDocumentCommand{\bO}{}{\mbf{O}}
\NewDocumentCommand{\bP}{}{\mbf{P}}
\NewDocumentCommand{\bQ}{}{\mbf{Q}}
\NewDocumentCommand{\bR}{}{\mbf{R}}
\NewDocumentCommand{\bS}{}{\mbf{S}}
\NewDocumentCommand{\bT}{}{\mbf{T}}
\NewDocumentCommand{\bU}{}{\mbf{U}}
\NewDocumentCommand{\bV}{}{\mbf{V}}
\NewDocumentCommand{\bW}{}{\mbf{W}}
\NewDocumentCommand{\bX}{}{\mbf{X}}
\NewDocumentCommand{\bY}{}{\mbf{Y}}
\NewDocumentCommand{\bZ}{}{\mbf{Z}}

\NewDocumentCommand{\balpha}{}{\mbf{\alpha}}
\NewDocumentCommand{\bbeta}{}{\mbf{\beta}}
\NewDocumentCommand{\bchi}{}{\mbf{\chi}}
\NewDocumentCommand{\bdelta}{}{\mbf{\delta}}
\NewDocumentCommand{\bepsilon}{}{\mbf{\epsilon}}
%\NewDocumentCommand{\beta}{}{\mbf{\eta}}		<--- \beta is already a symbol
\NewDocumentCommand{\bgamma}{}{\mbf{\gamma}}
\NewDocumentCommand{\biota}{}{\mbf{\iota}}
\NewDocumentCommand{\bkappa}{}{\mbf{\kappa}}
\NewDocumentCommand{\blambda}{}{\mbf{\lambda}}
\NewDocumentCommand{\bmu}{}{\mbf{\mu}}
\NewDocumentCommand{\bnu}{}{\mbf{\nu}}
\NewDocumentCommand{\bomega}{}{\mbf{\omega}}
\NewDocumentCommand{\bphi}{}{\mbf{\phi}}
\NewDocumentCommand{\bpi}{}{\mbf{\pi}}
\NewDocumentCommand{\bpsi}{}{\mbf{\psi}}
\NewDocumentCommand{\brho}{}{\mbf{\rho}}
\NewDocumentCommand{\bsigma}{}{\mbf{\sigma}}
\NewDocumentCommand{\btau}{}{\mbf{\tau}}
\NewDocumentCommand{\btheta}{}{\mbf{\theta}}
\NewDocumentCommand{\bupsilon}{}{\mbf{\upsilon}}
\NewDocumentCommand{\bvarepsilon}{}{\mbf{\varepsilon}}
\NewDocumentCommand{\bvarpi}{}{\mbf{\varpi}}
\NewDocumentCommand{\bvarphi}{}{\mbf{\varphi}}
\NewDocumentCommand{\bvarrho}{}{\mbf{\varrho}}
\NewDocumentCommand{\bvarsigma}{}{\mbf{\varsigma}}
\NewDocumentCommand{\bvartheta}{}{\mbf{\vartheta}}
\NewDocumentCommand{\bxi}{}{\mbf{\xi}}
\NewDocumentCommand{\bzeta}{}{\mbf{\zeta}}

\NewDocumentCommand{\bDelta}{}{\mbf{\Delta}}
\NewDocumentCommand{\bGamma}{}{\mbf{\Gamma}}
\NewDocumentCommand{\bLambda}{}{\mbf{\Lambda}}
\NewDocumentCommand{\bOmega}{}{\mbf{\Omega}}
\NewDocumentCommand{\bPhi}{}{\mbf{\Phi}}
\NewDocumentCommand{\bPi}{}{\mbf{\Pi}}
\NewDocumentCommand{\bPsi}{}{\mbf{\Psi}}
\NewDocumentCommand{\bSigma}{}{\mbf{\Sigma}}
\NewDocumentCommand{\bTheta}{}{\mbf{\Theta}}
\NewDocumentCommand{\bUpsilon}{}{\mbf{\Upsilon}}
\NewDocumentCommand{\bXi}{}{\mbf{\Xi}}



==> experiments.tex <==
\section{experiments}

In this section we demonstrate the consistency of the proposed estimator using several experiments. In the first experiment we consider a two-coordinate system $XY$ with dimensions $d_X=d_Y=1$. We choose a uniform distribution for $X$ within $[0,4]$, and r.v $Y$ is just a noisy version of $X$, and is defined as follows 

\begin{equation}
	Y\defeq X+N
\end{equation}
where $N$ has a normal density with the mean $\mu=0$ and standard deviation $\sigma=0.3$. 
The first experiment, shown in figure \ref{MI2cor} evaluates the the renyi mutual information function defined in \eqref{mutual_information} for $X,Y$. In this experiment we take $\alpha=0.3$.
We consider the number of iterations between 100 and 10000, and in each case we repeat the experiment 20 times and compute the mean squared error of the estimator. Three different values are chosen for $k$; 5, 10 and 20, and results are compared in the figure.


\begin{figure}\label{MI2cor}
	\centering
	\includegraphics[width=12cm]{MI2cor.png}
	\caption{Mean squared error as a function of the numbers of samples, for mutual information measure for a two-coordinate system.}
\end{figure}


In the second experiment we consider a three coordinate system $XYZ$, each with dimension $d=1$. We consider a Markov chain statistics for $X$,$Y$, and $Z$. We choose a uniform distribution for $X$ within $[0,4]$, and r.v $Y$ is a noisy version of $X$. Similarly, $Z$ is obtained by adding a normal noise $N_2$ to $Y$. 
\begin{equation}
	X\longrightarrow Y\longrightarrow Z\nonumber
\end{equation}

\begin{align}
Y\defeq X+N_1\nonumber\\
Z\defeq Y+N_2
\end{align}
where $N_1$ and $N_2$ have normal densities both with mean $\mu=0$ and standard deviation $\sigma=0.3$. 
For this experiment which is shown in figure \ref{MI2cor}  we evaluate the the renyi mutual information function between three systems $X$, $Y$ and $Z$. We also set $\alpha=0.3$.

Similarly we take the number of iterations between 100 and 10000, and in each case we repeat the experiment 20 times and compute the mean squared error of the estimator. Three different values are chosen for $k$; 5, 10 and 20, and results are compared in the figure.

\begin{figure}\label{3coordinate}
	\centering
	\includegraphics[width=12cm]{3coordinate.png}
	\caption{Mean squared error as a function of the numbers of samples, for mutual information measure for a three-coordinate system.}
\end{figure}

==> introduction.tex <==
\section{Introduction}

Shannon entropy, mutual information, and the Kullback-Leibler (KL) divergence are major information theoretic measures. Shannon entropy can measure diversity or uncertainty of samples, while KL-divergence is a measure of dissimilarity, and mutual information is a measure of dependency between two  probability distributions \cite{cover2012}. R\'{e}nyi  proposed a divergence measure which generalizes KL-divergence \cite{rrnyi1961}. F-divergence is another general family which is also well studied, and comprises many important divergence measures such as KL-divergence, total variation distance, and $\alpha$-divergence \cite{ali}. 
These measures have wide range of applications in information and coding theory, statistics and machine learning \cite{cover2012,moon2014,structure2016}. 


A major class of estimators for these measures is called non\hyp parametric, for which minimal assumptions on the density functions are considered in contrast to parametric estimators. An approach used for this class is plug-in estimation, in which we find an estimate of a distribution function and then plug it in the measure function. $k$-Nearest Neighbor ($K$-NN) and Kernel Density Estimator (KDE) methods are examples of this approach. Another approach is direct estimation, in which we find a relationship between the measure function and a functional in Euclidean space. 
In a seminal work in 1959, Beardwood et al derived the asymptotic behavior of the weighted functional of minimal graphs such as $K$-NN and TSP of $N$ i.i.d random points \cite{beardwood1959shortest}. They showed that the sum of weighted edges of these graphs converges to the integral of a weighted density function, which can be interpreted as R\'{e}nyi entropy. Since then, this work has been of great interest in signal processing and machine learning communities. Yet the extension to R\'{e}nyi divergence and f-divergences has remained an open question. Moreover, among various estimators of information measures, developing accurate and computationally tractable approaches has been often a challenge. Therefore, for  practical and computational reasons, direct graphical algorithms have been under attention in the literature including this work.

In this work, we propose an estimation method for R\'{e}nyi and f-divergences based on a direct graph estimation method. We show that given two sample sets $X$ and $Y$ with respective densities of $f_1$ and $f_2$, and the $k$-nearest neighbor ($k$-NN) graph of $Y$ in the joint data set $(X,Y)$, the average powered ratio of the number of $X$ points to the number of $Y$ points among all $k$-NN points converges to the R\'{e}nyi divergence. Using this fact, we design a consistent estimator for the R\'{e}nyi and f-divergences. 



Unlike most distance-based divergence estimators, our proposed estimator can use non-Euclidean metrics,
which makes this estimator appealing in many information theoretic and machine learning applications. 
Our estimator requires no boundary correction, and surprisingly, the boundary issues do not show up. This is because the proposed estimator automatically cancels the extra bias of the boundary points in the ratio of nearest neighbor points.
Our approach is also more computationally tractable than other estimators, with a time complexity of $O(kN\log N)$, required to construct the $k$-NN graph \cite{vaidya1989}. For example for $k=N^{1/{d+1}}$ we get the complexity of $O(N^{(d+2)/(d+1)}\log N)$. 
We show that for the class of $\gamma$-H\"{o}lder smooth functions, the estimator achieves the MSE rate of $O(N^{-2\gamma/(\gamma+d)})$.  Furthermore, by using the theory of optimally weighted ensemble estimation \cite{Kevin16,structure2016}, for density functions with continuous and bounded derivatives of up to the order $d$, and some extra conditions at the support set boundary, we derive an ensemble estimator that achieves the optimal MSE rate of $O(1/N)$, which is independent of the dimension.
Finally, the current work is an important step towards extending the direct estimation method studied in \cite{yukich} to more general information theoretic measures. 


Several previous works have investigated an estimator for a particular type of divergence measures. $k$-NN \cite{poczos2011}, KDE \cite{Poczos2014_2}, and histogram \cite{wang2009} estimators  are among the studied plug-in estimators for the f-divergence family. In general, most of these estimators suffer from several restrictions such as lack of analytic convergence rates, or high computational complexity. 

Recent works have focused on the MSE convergence rates for plug-in divergence estimators, such as KDE. Singh and P\'{o}czos proposed estimators for general density functionals and  R\'{e}nyi divergence, based on the kernel density plug-in estimator \cite{Poczos2014_2}, which can achieve the convergence rate of $O(1/N)$ when the densities are at least $d$ times differentiable. 
In a similar approach, Kandasamy et al  proposed another KDE-based estimator for general density functionals and divergence measures, which can achieve the convergence rate of $O(1/N)$ when the densities are at least $d/2$ differentiable \cite{kandasamy}.

Moon et al proposed simple kernel density plug-in estimators using weighted ensemble methods to improve the rate \cite{Kevin16}. The proposed estimator can achieve the convergence rate when the densities are at least
$(d+1)/2$ times differentiable. 
The main drawback of these estimators is handling the bias at the support set boundary. For example, using the estimators proposed in \cite{Poczos2014_2,kandasamy} requires knowledge of the densities' support set and numerous computations at the support boundary, which become complicated when the dimension increases. To circumvent this issue, Moon et al \cite{Kevin16} assumed smoothness conditions at the support set boundary, which may not always be true in practice. In contrast, our basic estimator does not require any smoothness assumptions on the support set boundary although our ensemble estimator does. Regarding the algorithm time complexities, our estimator spends $O(kN\log N)$ time versus the time complexity of KDE based estimators which spend $O(N^2)$ time.

A rather different method for estimating f-divergences is suggested by Nguyen et al \cite{Nguyen}, which is based on a variational representation of f-divergences that connects the estimation problem to a convex risk minimization problem. This approach achieves the parametric rate of $O(1/N)$ when the likelihood ratio is at least $d/
2$ times differentiable. However, the algorithm's time complexity is even worse than $O(N^2)$.




